Proposition-Level Clustering for Multi-Document Summarization

Text clustering methods were traditionally incorporated into multi-document summarization (MDS) as a means for coping with considerable information repetition. Particularly, clusters were leveraged to indicate information saliency as well as to avoid redundancy. Such prior methods focused on clustering sentences, even though closely related sentences usually contain also non-aligned parts. In this work, we revisit the clustering approach, grouping together sub-sentential propositions, aiming at more precise information alignment. Specifically, our method detects salient propositions, clusters them into paraphrastic clusters, and generates a representative sentence for each cluster via text fusion. Our summarization method improves over the previous state-of-the-art MDS method in the DUC 2004 and TAC 2011 datasets, both in automatic ROUGE scores and human preference.

==> tables/factuality.tex <==
\begin{table}[!tbp]
\centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|}
       & \textbf{system} & \textbf{Factuality}  \\ \hline
   \multirow{2}{*}{\rotatebox[origin=c]{90}{TAC}}
    & PG-MMR & 85.45  \\
      & ProCluster\textsubscript{abs} & 73.59   \\
    
      
   

    \specialrule{2.5pt}{1pt}{1pt}
    \multirow{2}{*}{\rotatebox[origin=c]{90}{DUC}}  
        & PG-MMR  & 86.53  \\
      & ProCluster\textsubscript{abs}  & 70.55  \\
    
     
    


    
    \end{tabular}}
    \caption{Factuality results by FactCC (TAC 2011 \& DUC 2004)}
    \label{tab_ablation}
    
\end{table}

==> tables/proposition_motivation.tex <==
\begin{table}[t]
\begin{scriptsize}

\begin{tabular}[t]{|p{2.89in}|}
\hline
\\[0.1mm]
\textbullet\, \textcolor{blue}{\textit{The trial opened Thursday of 29}} \textcolor{black}{mostly Moroccan} \textcolor{blue}{\textit{suspects charged with involvement in the 2004 Madrid train bomb attacks}}\textcolor{black}{, which killed 191 people and injured 1,824 in the worst terror strike to hit Spain.}
 \\[7.8mm]                        
\textbullet\, \textcolor{blue}{\textit{Of the 29 people who go on trial Thursday for the March 2004 Madrid train bombings}}\textcolor{black}{, seven face some 40,000 years in jail if found guilty.}
 \\[4.8mm]

\textbullet\,\textcolor{black}{But the man, Rabei Osman Sayed Ahmed -- expected to be the first of} \textcolor{blue}{\textit{29 defendants to take the stand when the bombing trial begins Thursday in Madrid}}\textcolor{black}{~-- also said in the recordings that the attack was carried out according to his plan.}
 \\[3.8mm] 

\hline

\end{tabular}

\end{scriptsize}
\caption{An example of a cluster of \textcolor{blue}{\textit{propositions}}, shown within their source sentence \textcolor{black}{context}, from TAC 2011 (topic D1103). Clustering these as sentences would yield noisy unaligned information, however grouping together only the marked propositions keeps information alignment clean.}
\label{tab:motivation_cluster}
\vspace{-0.15in}
\end{table}


